Private Queries on Public Certificate Transparency Data

Despite increasing advancements in today's information exchange infrastructure, the preservation of user data and privacy still remains a problem. Both insecure baselines and secure solutions leak user data. For example, Certificate Transparency (CT) promises significant security improvements to existing Public Key Infrastructure solutions that up-to-now have solely relied on the Certificate Authority hierarchy. CT provides a robust auditing layer and transparency solution to quickly detect such compromises, but introduces the requirement that client browsers interact with third-party servers when validating a site certificate. In the existing CT system, these requests leak information about each user's browsing habits to the hosting server. It is not a stretch to think that this valuable data could be collected and exploited, as corporations and governments have plenty of financial and political incentive to do so. In this project, we seek to address this problem by using an oblivious file sharing system with strong anonymity properties, to provide a more scalable, performant solution to privacy-preserving queries.

==> src/title.tex <==
\newlength{\rulewidth}
\setlength{\rulewidth}{2.5in}
\newlength{\ruleheight}
\setlength{\ruleheight}{0.5pt}

\begin{titlepage}
\begin{addmargin}{0.45in}

    \begin{center}
        \rule{\linewidth}{\ruleheight}
        \vspace*{2ex}

        \makeatletter
        \begin{LARGE}
            \textsf{\textbf{\@title}}
        \end{LARGE}
        \\ [3ex]
        \begin{large}
            \@author
        \end{large}
        \makeatother

        \vspace*{2ex}
        \rule{\linewidth}{\ruleheight}
    \end{center}

    \vspace*{2ex}
    \begin{center}
        \begin{large}
            \textsf{\textbf{Research Project}}
        \end{large}
    \end{center}

    \begin{small}
    \noindent
    Submitted to the Department of Electrical Engineering and Computer Sciences, University of California at Berkeley, in partial satisfaction of the requirements for the degree of \textsf{\textbf{Master of Science, Plan II}}.
    
    \vspace*{5ex}
    \noindent
    Approval for the Report and Comprehensive Examination:
    \end{small}

    \vspace*{2ex}
    \begin{center}
        \textsf{\textbf{Committee}}

        \begin{small}
            \vspace*{7ex}
            \rule{\rulewidth}{\ruleheight} \\
            \researchadvisor \\
            Research Advisor
    
            \vspace*{5ex}
            \rule{\rulewidth}{\ruleheight} \\
            (Date)
    
            \vspace*{5ex}
            \(\star\; \star\; \star\; \star\; \star\; \star\; \star\)
    
            \vspace*{7ex}
            \rule{\rulewidth}{\ruleheight} \\
            \secondreader \\
            Second Reader
    
            \vspace*{5ex}
            \rule{\rulewidth}{\ruleheight} \\
            (Date)
        \end{small}
    \end{center}
\afterpage{\blankpage}

\end{addmargin}
\end{titlepage}
